Dyport: Dynamic Importance-based Hypothesis Generation Benchmarking Technique

This paper presents a novel benchmarking framework Dyport for evaluating biomedical hypothesis generation systems. Utilizing curated datasets, our approach tests these systems under realistic conditions, enhancing the relevance of our evaluations. We integrate knowledge from the curated databases into a dynamic graph, accompanied by a method to quantify discovery importance. This not only assesses hypothesis accuracy but also their potential impact in biomedical research which significantly extends traditional link prediction benchmarks. Applicability of our benchmarking process is demonstrated on several link prediction systems applied on biomedical semantic knowledge graphs. Being flexible, our benchmarking system is designed for broad application in hypothesis generation quality verification, aiming to expand the scope of scientific discovery within the biomedical research community. Availability and implementation: Dyport framework is fully open-source. All code and datasets are available at: https://github.com/IlyaTyagin/Dyport

==> preface.tex <==
% This section allows us to modify preloaded package properties
\makeatletter
% These magic runes make comment's appear inline
% These also need to be above the other magic runes
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
\usepackage{regexpatch}
\xpatchcmd{\@todo}{\setkeys{todonotes}{#1}}{\setkeys{todonotes}{inline,#1}}{}{}

% These magic runes make the new changes package work with comments
\usepackage{comment}
\let\wfs@comment@comment\comment
\let\comment\@undefined
\usepackage{changes}
\let\wfs@changes@comment\comment
\let\comment\@undefined
\newcommand\comment{%
    \ifthenelse{\equal{\@currenvir}{comment}}
    {\wfs@comment@comment}
    {\wfs@changes@comment}%
}
\makeatother

% Typical preloader time

\usepackage{amsmath}
\usepackage{hyperref}
\usepackage{enumitem}
\usepackage{multirow}
\usepackage{outlines}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage{float}
\usepackage{nicefrac}
\usepackage{url}
\usepackage{booktabs}
\usepackage{listings}
\usepackage{subcaption}
\lstset{
  basicstyle=\ttfamily,
  columns=fullflexible,
  frame=single,
  breaklines=true,
  tabsize=2,
  breakautoindent=true,
}

% Changes Authors
\definechangesauthor[name="Ilya Tyagin", color=cyan]{it}
\definechangesauthor[name="Ilya Safro", color=red]{is}


\newcommand{\sysname}{Dyport }

% These are shortcuts for leaving specific changes comments
\newcommand{\note}[2]{\added[id=#1, comment={#2}]{}}

% ITyagin's add, delete replace
\newcommand{\Ait}[1]{\added[id=it]{#1}}
\newcommand{\Dit}[1]{\deleted[id=it]{#1}}
\newcommand{\Rit}[2]{\replaced[id=it]{#1}{#2}}

% ISafro's add, delete, replace
\newcommand{\Ais}[1]{\added[id=is]{#1}}
\newcommand{\Dis}[1]{\deleted[id=is]{#1}}
\newcommand{\Ris}[2]{\replaced[id=is]{#1}{#2}}

% THIS ALLOWS FOR CONDITIONAL COMMENTS
%\newif\ifthesis
% Comment/ un-comment as needed
%\thesisfalse
%\thesistrue

\newif\ifthesis
\thesistrue % use false for AAAI, true for full thesis

% % Comment out a block of text for KDD (but keep for thesis) with this syntax:
% \ifthesis
% % <Text to comment out>
% \else
% % <Optional replacement for KDD Version>
% \fi

%\thesisfalse
%\thesistrue

% These magic runes make everything denser

\setlength{\textfloatsep}{3pt}
\setlength{\floatsep}{3pt}
\setlength{\belowdisplayskip}{3pt} \setlength{\belowdisplayshortskip}{3pt}
\setlength{\abovedisplayskip}{3pt} \setlength{\abovedisplayshortskip}{3pt}
